Transformer-based Network for RGB-D Saliency Detection

RGB-D saliency detection integrates information from both RGB images and depth maps to improve prediction of salient regions under challenging conditions. The key to RGB-D saliency detection is to fully mine and fuse information at multiple scales across the two modalities. Previous approaches tend to apply the multi-scale and multi-modal fusion separately via local operations, which fails to capture long-range dependencies. Here we propose a transformer-based network to address this issue. Our proposed architecture is composed of two modules: a transformer-based within-modality feature enhancement module (TWFEM) and a transformer-based feature fusion module (TFFM). TFFM conducts a sufficient feature fusion by integrating features from multiple scales and two modalities over all positions simultaneously. TWFEM enhances feature on each scale by selecting and integrating complementary information from other scales within the same modality before TFFM. We show that transformer is a uniform operation which presents great efficacy in both feature fusion and feature enhancement, and simplifies the model design. Extensive experimental results on six benchmark datasets demonstrate that our proposed network performs favorably against state-of-the-art RGB-D saliency detection methods.

==> experi.tex <==

%%%%%%%%% ABSTRACT

\section{Experiments}

\begin{table*}[ht]
  \centering \caption{Ablation Study on our proposed transformer-based network. We highlight the best result in each column in 
    \underline{\textbf{bold}}.}
 % \underline{\textbf{red}}.}
\centering 
\resizebox{0.75\textwidth}{!}{%
    \begin{tabular}{c|cccc|cccc|cccc}
\toprule
& \multicolumn{4}{c|}{NJUD}      & \multicolumn{4}{c|}{STERE}     & \multicolumn{4}{c}{SIP} \\

model
& MAE   & $F_m$  & $S_m$    & $E_m$    
& MAE   & $F_m$  & $S_m$    & $E_m$     
& MAE   & $F_m$  & $S_m$    & $E_m$  \\
\hline
B 
& 0.048 & 0.866 & 0.888 & 0.918 
& 0.052 & 0.848 & 0.870 & 0.919 
& 0.063 & 0.832 & 0.857 & 0.902 \\

B+TFUM 
& 0.041 & 0.878 & 0.904 & 0.919 
& 0.046 & 0.861 & 0.891 & 0.922 
& 0.059 & 0.845 & 0.870 & 0.908 \\

Ours\_e 
& \underline{\textbf{0.038}}  & \underline{\textbf{0.889}}  & \underline{\textbf{0.912}}  & \underline{\textbf{0.928}}  
& 0.042  & \underline{\textbf{0.875}}  & \underline{\textbf{0.900}}  & \underline{\textbf{0.933}}  
& \underline{\textbf{0.051}}  & \underline{\textbf{0.869}}  & \underline{\textbf{0.884}}  & \underline{\textbf{0.919}}  \\

Ours\_s
& \underline{\textbf{0.038}}  & 0.885  & 0.909  & 0.926  
& \underline{\textbf{0.041}}  & 0.874  & 0.899  & \underline{\textbf{0.933}}  
& \underline{\textbf{0.051}}  & 0.865  & 0.882  & 0.917 \\
\bottomrule  
    \end{tabular}%
  \label{tab:abtab1}%
}
  \vspace{-0.1cm} 
\end{table*}%


\begin{table*}[!ht]
  \centering
  \caption{
 % Comparison of setting different stacks for our transformer-based fusion model with the entangled architecture. We highlight the best result in each column in \underline{\textbf{red}.
    Comparison of setting different T for the entangled architecture. We highlight the best result in each column in \underline{\textbf{bold}}.
  }
\centering 
\resizebox{0.75\textwidth}{!}{%
    \begin{tabular}{c|cccc|cccc|cccc}
\toprule
& \multicolumn{4}{c|}{NJUD}      
& \multicolumn{4}{c|}{STERE}     
& \multicolumn{4}{c}{SIP} \\

    model\_name 
    & MAE   & $F_m$  & $S_m$    & $E_m$    
    & MAE   & $F_m$  & $S_m$    & $E_m$    
    & MAE   & $F_m$  & $S_m$    & $E_m$ \\
\hline
\iffalse
    T=0 
    & 0.0412  & 0.8778  & 0.9043  & 0.9187  
    & 0.0455  & 0.8612  & 0.8912  & 0.9223  
    & 0.0585  & 0.8448  & 0.8704  & 0.9079  \\
    \fi
    
        T=0 
    & 0.041  & 0.878  & 0.904  & 0.919  
    & 0.046  & 0.861  & 0.891  & 0.922  
    & 0.059  & 0.845  & 0.870  & 0.908  \\
    
    \iffalse
    T=2 
    & 0.0383  & 0.8861  & 0.9092  & 0.9263  
    & 0.0438  & 0.8720  & 0.8966  & 0.9294  
    & 0.0522  & 0.8598  & 0.8786  & 0.9144  \\
    \fi
    
    T=2 
    & 0.038  & 0.886  & 0.909  & 0.926  
    & 0.044  & 0.872  & 0.897  & 0.929  
    & 0.052  & 0.860  & 0.879  & 0.914  \\
    
    \iffalse
    T=4 
    & 0.0382  & \underline{\textbf{0.8891}}  & 0.9121  & 0.9283  
    & \underline{\textbf{0.0415}}  & \underline{\textbf{0.8750}}  & 0.9004  & \underline{\textbf{0.9328}}  
    & 0.0511  & \underline{\textbf{0.8687}}  & \underline{\textbf{0.8842}}  & \underline{\textbf{0.9188}}  \\
    \fi
    
     T=4 
    & 0.038  & \underline{\textbf{0.889}}  & 0.912  & 0.928 
    & \underline{\textbf{0.042}}  & \underline{\textbf{0.875}}  & 0.900  & \underline{\textbf{0.933}}  
    & 0.051  & \underline{\textbf{0.869}}  & \underline{\textbf{0.884}}  & \underline{\textbf{0.919}}  \\
    
    \iffalse
    T=5 
    & \underline{\textbf{0.0368}}  & 0.8874  & \underline{\textbf{0.9128}}  & \underline{\textbf{0.9295}}  
    & 0.0421  & 0.8721  & \underline{\textbf{0.9011}}  & 0.9300  
    & \underline{\textbf{0.0504}}  & 0.8668  & 0.8832  & 0.9173  \\
    \fi
    
    T=5 
    & \underline{\textbf{0.037}}  & 0.887  & \underline{\textbf{0.913}}  & \underline{\textbf{0.930}}  
    & \underline{\textbf{0.042}}  & 0.872  & \underline{\textbf{0.901}}  & 0.930  
    & \underline{\textbf{0.050}}  & 0.867  & 0.883  & 0.917  \\
    
 \iffalse
\hline

    T=0 
& 0.0412  & 0.8778  & 0.9043  & 0.9187  
& 0.0455  & 0.8612  & 0.8912  & 0.9223  
& 0.0585  & 0.8448  & 0.8704  & 0.9079  \\

    T=2 
& 0.0393  & 0.8864  & 0.9089  & 0.9239  
& 0.0430  & 0.8706  & 0.8972  & 0.9306  
& 0.0533  & 0.8553  & 0.8779  & 0.9128  \\

    T=4 
& 0.0385  & 0.8854  & 0.9089  & 0.9262  
& 0.0413  & 0.8737  & 0.8993  & 0.9328  
& 0.0512  & 0.8646  & 0.8818  & 0.9172  \\

    T=5 
& 0.0369  & 0.8869  & 0.9139  & 0.9270  
& 0.0423  & 0.8728  & 0.8983  & 0.9308  
& 0.0534  & 0.8619  & 0.8797  & 0.9148  \\
\fi
\bottomrule
    \end{tabular}%
}
  \label{tab:abtab2}%
    \vspace{-0.1cm} 
\end{table*}%


\iffalse
In this section, we evaluate our method and present the experimental results. 
First, we introduce the benchmark datasets and some implementation details of our network architecture. 
Then, we discuss the effectiveness of our method by comparison with the state-of-art methods
and the ablation study.
\fi

\subsection{Datasets and Evaluation Metrics}
We evaluate our proposed method on six widely used RGB-D saliency datasets including
NJUD~\cite{ju2014depth},  
NLPR~\cite{peng2014rgbd},
%LFSD~\cite{li2014saliency},
STERE~\cite{niu2012leveraging},
RGBD135~\cite{cheng2014depth},
SIP~\cite{fan2019rethinking},
and DUT-D~\cite{piao2019depth}.
We use the selected 800 images from DUT-D, 1485 images from NJUD and 700 images from NLPR
as in~\cite{piao2019depth} for training our RGB-D saliency detection model.
We then evaluate our model on the remaining images in these three datasets and the other three datasets. 

We adopt four widely used evaluation metrics for quantitative evaluation
including F-measure ($F_m$)~\cite{achanta2009frequency}, mean absolute error (MAE)~\cite{borji2015salient}, 
S-measure ($S_m$)~\cite{fan2017structure} and E-measure ($E_m$)~\cite{fan2018enhanced}.
In this paper, we report the mean F-measure value with the adaptive threshold as $F_m$.
For MAE, the lower value means the method is better, 
while for all other metrics, the higher value means the method is better.

\subsection{Implementation Details}
We apply PyTorch toolbox for implementation using one GeForce RTX 1080Ti GPU with 11 GB memory.
The backbone of our method is the pretrained VGG16~\cite{simonyan2014very} network.
The input RGB images and depth images are all resized to $ 256 \times 256$.
We train our method for 150k iterations by ADAM optimizer~\cite{kingma2014adam}. 
The initial learning rate, the batch size, the number of channel $c$ and the number of stacks in transformer-based fusion module $T$ are set to 1e-4, 6, 64 and 4.
During evaluation, the output prediction map of the last transformer-based fusion stack is used as the final saliency prediction map.

\subsection{Comparison with state-of-the-art methods}
To verify the effectiveness of our proposed transformer-based network for RGB-D saliency detection,
we compare our performance with eleven state-of-art RGB-D saliency detection methods
including: 
DANet~\cite{zhao2020single},
%SSF~\cite{zhang2020select},
S2MA~\cite{liu2020learning},
ICNET~\cite{li2020icnet},
CMWNet~\cite{ling2020cross},
%CMMS~\cite{li2020rgb} (?),
DMRA~\cite{piao2019depth}, 
CPFP~\cite{zhao2019contrast}, TANet~\cite{chen2019three}, 
MMCI~\cite{chen2019multi}, PCANet~\cite{chen2018progressively},
A2dele~\cite{piao2020a2dele} 
CTMF~\cite{han2017cnns}.
The quantitative results are shown in Table~\ref{tab:exp_tab1}.
%According to the proportion of each testing set to all testing sets, the results on all datasets are weighted and summed to obtain an overall performance evaluation, which is listed in the row ?Ave-Metric?
%To better present the overall performance of each method among all the testing datasets,
To present the overall performance,
we show ``Avg." which calculates the mean performance across all testing datasets, and ``weight-Avg." which calculates the weighted mean by the proportion of each testing set to all.

%The comparisons in Table~\ref{tab:exp_tab1} 
It demonstrates that our method with either straightforward or entangled architecture for transformer-based fusion module generally performs favorably against all the listed state-of-art methods. 
%Meanwhile, our result of using entangled architecture is slightly better than our result of straightforward architecture since it may focus more on exploring complementary information between two modalities. 
%Meanwhile, our straightforward and entangled fusion architectures achieve similar performance 
%even though they fuse multi-scale multi-modal features in different ways.
Meanwhile, our straightforward and entangled fusion architectures achieve similar performance
indicates that straightforward fusion can also extract complementary information
from multi-scale multi-modal features. 
Our result may be slightly lower than CMWNet and S2MA on few metrics, 
%in RGBD135 and STERE datasets,
but we perform a better overall performance than these two methods.
\iffalse
A2dele is also slightly better than ours on STERE dataset on $F_m$. 
However, since it does not use depth data during testing, our method achieves much better performance than it on all other testing datasets.
\fi
Moreover, since we fuse features from all scales and modalities at one time and only use the transformer-based structure with the efficient attention for both feature fusion and update instead of designing diverse models,
the model size of our network is smaller than other two-steam methods with good performance as listed in Table~\ref{tab:exp_tab2}.
Our model size is still a little larger than A2dele and DANet, since A2dele only has RGB image as input to the network
and DANet uses one-steam network with two modalities as one input. 
%To better demonstrate the advantage of our method, 
We also present some qualitative examples in Fig.\ref{fig:exp1}.


\subsection{Ablation Study}

\begin{figure}[b] 
\centering
%\includegraphics[width=0.35\textwidth, height=0.35\textheight]{./im/tdm1.pdf}
\includegraphics[width=0.48\textwidth]{./im/ab1.pdf}
 \caption{Visual examples for ablation study.}
\label{fig:ab1}
  \vspace{-0.1cm} 
\end{figure} 

\textbf{Effectiveness of each transformer-based module.} To demonstrate the impact of our transformer-based feature update module and fusion module, we conducted our ablation study by evaluating the following subset models:
%\subsubsection{Transformer-based update and fusion}

1) B:  a simple fusion method without any transformer-based modules.
It can be considered as to set $f_{5m}=f_5$, $f_{4m} = f_{5m} + f_4$,
$ f_{3m} = f_{4m} +f_3$ for a simple multi-scale feature fusion on each modality branch.
And then it directly uses $f_{3m}^r + f_{3m}^d$ for multi-modal fusion to produce the saliency prediction map as the final output.

2) B+TFUM: a simple fusion method with only transformer-based feature update module to enhance features for each modality branch across scale, 
and combine the multi-modal features with a simple fusion way to produce the saliency prediction map as the final output.

3) Ours (B+TFUM+TFFM): our overall transformer-based network by further adding the transformer-based feature fusion module.
%The enhanced features from transformer-based feature update model are used for getting a simple initial fused feature as the initial query for our transformer-based fusion process. 
%These enhanced features from all scales and modalities are also used in our transformer-based fusion model for a simultaneous multi-scale multi-modal feature fusion. 

Our ablation study is evaluated on three RGB-D datasets and the result is showed in Table~\ref{tab:abtab1}.
We also include some visual examples in Fig.\ref{fig:ab1}.
It indicates that by adding our transformer-based feature update module, the saliency prediction of our simple fusion across two modalities can be improved due to the update across scales for each modality.
However, this simple fusion process is not suitable for various situations since it does not consider the global selection and fusion among features from all scales and modalities.
By further adding our transformer-based feature fusion module to simultaneously fuse all features, the performance can be further improved. 

\textbf{Effectiveness of $\bold{T}$.} We also discuss the chosen number of stacks in our transformer-based fusion module by conducting the experiments to set $T=0, 2, 4, 5$ for the fusion stacks in our overall transformer-based network
(by setting $T=0$ is equal to the model of B + TFUM).
We present the comparisons on three datasets with the entangled fusion in Table~\ref{tab:abtab2}. 
Since the initial fused feature from our transformer-based update module provides useful information related to saliency prediction for our transformer-based fusion module as the initial query. By setting different $T$ may not have a significant influence on the final result predicted by the output feature from the last stack, especially when $T$ is large enough.
However, using a small number of stacks may still affect the performance on some datasets such as the SIP dataset.
Considering both the performance and the efficiency of our model, we choose $T=4$ for our transformer-based network for RGB-D saliency detection. 
 
 
\iffalse
%\subsubsection{Number of stack for Transformer-based fusion}
Since we have a good initial as initial query to our transformer-based fusion,
the number of stack may not have significant influence to the final results.
However, by reducing the number of stacks may still affect the performance of some datasets.
Considering both the performance and the efficiency, we choose $T=4$. 
\fi

\iffalse
{\small
\bibliographystyle{ieee_fullname}
\bibliography{egbib}
}

\end{document}
\fi

